Order-Preserving Key Compression for In-Memory Search Trees

We present the High-speed Order-Preserving Encoder (HOPE) for in-memory search trees. HOPE is a fast dictionary-based compressor that encodes arbitrary keys while preserving their order. HOPE's approach is to identify common key patterns at a fine granularity and exploit the entropy to achieve high compression rates with a small dictionary. We first develop a theoretical model to reason about order-preserving dictionary designs. We then select six representative compression schemes using this model and implement them in HOPE. These schemes make different trade-offs between compression rate and encoding speed. We evaluate HOPE on five data structures used in databases: SuRF, ART, HOT, B+tree, and Prefix B+tree. Our experiments show that using HOPE allows the search trees to achieve lower query latency (up to 40\% lower) and better memory efficiency (up to 30\% smaller) simultaneously for most string key workloads.

==> art-eval.tex <==
\begin{adjustbox}{width=1.0\textwidth,totalheight=\textheight,keepaspectratio}

\begin{tabular}{cccc}

  \multicolumn{4}{c}
  {\includegraphics[width=\textwidth]{figures/ppt/legend_new.pdf}} \\

  & {\Large \textbf{Email}}
  & {\Large \textbf{Wiki}}
  & {\Large \textbf{URL}} \\

  %% ----------------------------------------------------------------

  {\rotatebox{90}{\hskip 1.2em \Large \textbf{Point vs. Memory}}}

  & \includegraphics[width=0.33\textwidth]{figures/ART/point/lat_mem_email_art_point.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/ART/point/lat_mem_wiki_art_point.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/ART/point/lat_mem_url_art_point.pdf} \\

  %% ----------------------------------------------------------------

  {\rotatebox{90}{\hskip 1.8em \Large \textbf{Range \& Insert}}}

  & \includegraphics[width=0.33\textwidth]{figures/ART/range/lat_email_art.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/ART/range/lat_wiki_art.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/ART/range/lat_url_art.pdf} \\

  %% ----------------------------------------------------------------

  %{\rotatebox{90}{\hskip 1.8em \Large \textbf{Trie Height}}}

  %& \includegraphics[width=0.33\textwidth]{figures/ART/point/height_email_art.pdf}

  %& \includegraphics[width=0.33\textwidth]{figures/ART/point/height_wiki_art.pdf}

  %& \includegraphics[width=0.33\textwidth]{figures/ART/point/height_url_art.pdf} \\

\end{tabular}

\end{adjustbox}


==> art-hot-btree-eval.tex <==
\begin{adjustbox}{width=\textwidth,totalheight=\textheight,keepaspectratio}

\newcommand{\mysize}{0.33}

\begin{tabular}{ccccc}

  \multicolumn{5}{c}
  {\includegraphics[width=1.15\textwidth]{figures/ppt/legend_new2.pdf}} \\

  &
  & {\LARGE \textbf{Email}}
  & {\LARGE \textbf{Wiki}}
  & {\LARGE \textbf{URL}} \\

  %% ----------------------------------------------------------------

  \multirow{2}{*}{\rotatebox{90}{\LARGE \textsc{\textbf{\art}}}}

  & {\rotatebox{90}{\hskip 1.2em \Large \textbf{Point vs. Memory}}}

  & \includegraphics[width=\mysize\textwidth]{figures/ART/point/lat_mem_email_art_point.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/ART/point/lat_mem_wiki_art_point.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/ART/point/lat_mem_url_art_point.pdf} \\

  & {\rotatebox{90}{\hskip 1.8em \Large \textbf{Range \& Insert}}}

  & \includegraphics[width=\mysize\textwidth]{figures/ART/range/lat_email_art.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/ART/range/lat_wiki_art.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/ART/range/lat_url_art.pdf} \\

  \hlineB{2} \\

  %% ----------------------------------------------------------------

  \multirow{2}{*}{\rotatebox{90}{\LARGE \textsc{\textbf{\hot}}}}

  & {\rotatebox{90}{\hskip 1.2em \Large \textbf{Point vs. Memory}}}

  & \includegraphics[width=\mysize\textwidth]{figures/hot/point/lat_mem_email_hot.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/hot/point/lat_mem_wiki_hot.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/hot/point/lat_mem_url_hot.pdf} \\

  & {\rotatebox{90}{\hskip 1.8em \Large \textbf{Range \& Insert}}}

  & \includegraphics[width=\mysize\textwidth]{figures/hot/range/lat_email_hot.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/hot/range/lat_wiki_hot.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/hot/range/lat_url_hot.pdf} \\

  \hlineB{2} \\

  %% ----------------------------------------------------------------

  \multirow{2}{*}{\rotatebox{90}{\LARGE \textsc{\textbf{\bplustree}}}}

  & {\rotatebox{90}{\hskip 1.2em \Large \textbf{Point vs. Memory}}}

  & \includegraphics[width=\mysize\textwidth]{figures/btree/point/lat_mem_email_btree_point.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/btree/point/lat_mem_wiki_btree_point.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/btree/point/lat_mem_url_btree_point.pdf} \\

  & {\rotatebox{90}{\hskip 1.8em \Large \textbf{Range \& Insert}}}

  & \includegraphics[width=\mysize\textwidth]{figures/btree/range/lat_email_btree.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/btree/range/lat_wiki_btree.pdf}

  & \includegraphics[width=\mysize\textwidth]{figures/btree/range/lat_url_btree.pdf}

\end{tabular}

\end{adjustbox}


==> btree-eval.tex <==
\begin{adjustbox}{width=1.0\textwidth,totalheight=\textheight,keepaspectratio}

\begin{tabular}{cccc}

%   \multicolumn{4}{c}
%   {\includegraphics[width=\textwidth]{figures/ppt/legend_new.pdf}} \\

  & {\Large \textbf{Email}}
  & {\Large \textbf{Wiki}}
  & {\Large \textbf{Url}} \\

  %% ----------------------------------------------------------------

  {\rotatebox{90}{\hskip 1.2em \Large \textbf{Point vs. Memory}}}

  & \includegraphics[width=0.33\textwidth]{figures/btree/point/lat_mem_email_btree_point.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/btree/point/lat_mem_wiki_btree_point.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/btree/point/lat_mem_url_btree_point.pdf} \\

  %% ----------------------------------------------------------------

  {\rotatebox{90}{\hskip 1.8em \Large \textbf{Range \& Insert}}}

  & \includegraphics[width=0.33\textwidth]{figures/btree/range/lat_email_btree.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/btree/range/lat_wiki_btree.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/btree/range/lat_url_btree.pdf} \\

\end{tabular}

\end{adjustbox}


==> eval.tex <==
%% \section{Evaluation}
%% \label{sec:eval}

%% \section{Evaluation Steps}
%% \begin{enumerate}
%%     \item We first test the performance of encoders by looking at the compression rate, memory use, and average time to encode each character for different schemes
%%     \item Then we merge the encoders into different index trees to test the overall insert and lookup performance 
%% \end{enumerate}


%% \section{Experiment Setup \& Benchmarks}
%% \begin{align*}
%%     {\bf CPU:} &\text{Intel\textregistered Xeon\textregistered E5-2630 v4 CPUs @ 2.20GHz}\\
%%     {\bf DRAM:} & \\
%%     {\bf Cache:} & \text{256 KB L2-cache, 26 MB L3-cache}\\
%%     {\bf Disk:} & \\
%% \end{align*}

%% \begin{enumerate}
%%     \item Use YCSB-based microbenchmarks to mimic OLTP index workloads
%%     \item Use default workloads (read only) with Zipfian distributions
%%     \item Initialization phase: randomly select partial keys(2.5 million for email, 1.4 million for wiki, 25K for url) to generate encoders for different schemes
%%     \item Measurement phase: \\
%%         a. use all key-value pairs (25 million for email, 14 million for wiki, 25 million for url) to build index trees,  test insert performance\\
%%         b. execute 10 million key-value point and range queries, test lookup performance\\
%%     \item All experiments are single threaded without any network activity.
%% \end{enumerate}

%% \begin{align*}
%%     {\bf Evaluate\ schemes:} & \text{single, double, 3-gram, 4-gram, ALM}\\
%%     {\bf Dictionary\ Data\ Structure:} & \text{256-entry array, 256*256-entry array}\\
%%                                        & \text{3-layer huanchen optimized trie, 4-layer huanchen optimized trie, ART}\\
%%     {\bf Index\ Tree\ Types:} & \text{SuRF, Btree, ART, HOT}\\
%%     {\bf Key\ Types:} & \text{email, url, wiki titles}\\
%%     {\bf Value:} & \text{64-bit integer (tuple pointers)}\\
%%     {\bf Workloads:} & \text{Point query, Range query}
%% \end{align*}


%% \section{Encoder Evaluation}
%% \begin{figure}
%% \caption{Comparing the compression rate, latency, and memory for different Compression Schemes.}
%% \end{figure}
%% \begin{enumerate}
%%     \item Compression rate: 
    
%%     Compression rate is defined as the original string size over encoded string size. Higher compression rate indicates better compression performance.
    
%%     All compression schemes perform best on emails (compression rate higher than 1.6), reducing the string size by 30\%$\sim$60\% . This is not surprising because emails contain common patterns (@xxx.yyy) that are caught by the compression schemes to replace with short codes.

%%     \item Latency:
%%     The latency for single and double character are less than 10ns per character because the underlying array implementation ensures efficient lookup. For 3-gram, 4-gram, ALM, more complicated tree-based dictionary data structures are used. The encoder needs to step into more layers and introduce higher latency.
    
%%     ALM is much slower than other compression schemes because ALM stores variable-length boundaries. The height of its dictionary (ART) is changed as the sample size increases and more boundaries are introduced, while for 3-gram trie, 4-gram, we only need to step into 3 or 4 layers.

%%     \item Memory use:
%%     Single, double character have fixed dictionary size (256 entries for single character, 256 * 256 entries for double character). ALM needs 2 times memory compared with 3-Gram and 4-Gram.
%% \end{enumerate}


%% \section{Index tree evaluation}
%% \begin{figure}
%% \caption{Integrating compression schemes into Basic SuRF.}
%% \end{figure}

%% \subsection{SuRF}
%% \begin{enumerate}
%%     \item Double character scheme has best overall performance across all workloads in three datasets. It reduces memory by 10\% to 26\%. The most savings come from URL.  All three datasets have similar latency reduction (about 40\% for point queries and 33\% for range queries).
%%     \item Although ALM has small trie heights, it has worst performance because the memory and latency savings are offset by big dictionary and slow lookup.
%%     \item Double-character scheme has best compression rate on email dataset, but the memory reduction is minimum after merging into SuRF. This is because all savings come from the reduction of internal nodes. For emails, there are not many internal nodes before compression. Although more internal nodes are eliminated, the percentage of savings is less obvious because the leaf nodes that consume large portion of memory keep unchanged.
%% \end{enumerate}

%% \subsection{ART}
%% \begin{enumerate}
%%     \item Memory savings are not that obvious because ART stores keys optimistically. ART cannot take full advantage of our compression because nodes will skip partial keys to save memory. 
%%     \item 
%% \end{enumerate}

%% \subsection{BTree}
%% \begin{enumerate}
%%     \item The structure of B tree will not change after compression. Keys are not inlined. Each node stores pointers to the encoded keys.
%%     \item The memory use is reduced because encoded keys are smaller.
%%     \item For email and wiki, lookup latency reduces up to 20% because of better cache performance. Keys are smaller and more keys can fit in cache.
%%      \item For Url, all schemes reduce memory by about 25% but latency is increased. *This is because compressed urls are still long. And only part of those urls can be stored in the cache. There will still be many cache miss during lookup even if keys are compressed. So the latency will still be high.
%% \end{enumerate}

%% \subsection{HOT}
%% \begin{enumerate}
%%     \item Trie height are very similar for all schemes. (Why?)
%%     \item
%% \end{enumerate}


==> hot-eval.tex <==
\begin{adjustbox}{width=1.0\textwidth,totalheight=\textheight,keepaspectratio}

\begin{tabular}{cccc}

  \multicolumn{4}{c}
  {\includegraphics[width=\textwidth]{figures/ppt/legend_new.pdf}} \\

  & {\Large \textbf{Email}}
  & {\Large \textbf{Wiki}}
  & {\Large \textbf{URL}} \\

  %% ----------------------------------------------------------------

  {\rotatebox{90}{\hskip 1.2em \Large \textbf{Point vs. Memory}}}

  & \includegraphics[width=0.33\textwidth]{figures/hot/point/lat_mem_email_hot.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/hot/point/lat_mem_wiki_hot.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/hot/point/lat_mem_url_hot.pdf} \\

  %% ----------------------------------------------------------------

  {\rotatebox{90}{\hskip 1.8em \Large \textbf{Range \& Insert}}}

  & \includegraphics[width=0.33\textwidth]{figures/hot/range/lat_email_hot.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/hot/range/lat_wiki_hot.pdf}

  & \includegraphics[width=0.33\textwidth]{figures/hot/range/lat_url_hot.pdf} \\

\end{tabular}

\end{adjustbox}


==> ope_theory.tex <==
\section{Fast Order-Preserving Entropy Encoding}
\label{sec:ophe}

OPE model

Abstract model

Different heuristics
single, double, 3-gram, 4-gram, 
ALM, 
ALM + better equalize,
ALM + prefix code


OPE framework and implementation

Overview: block diagram

Implementation
SS: freq count, ss with fixed-size dict
CG: Dict, Hu-Tucker
DICT: array, specialized trie, ART
ENC: fast bit cat, SIMD, batch optimize

ALM-improved: ss suffix


Integration

Performance model
index category


Evaluation

Micro
main result: cpr, latency, dict mem, add ALM-improved, x align
build time (breakdown): stacked bar, 2 sets
sample size vs. cpr rate
binary search vs. specialized trie
batch insert vs. insert performance gain
ALM suffix benefit

Applied to search trees
pick the best ALM
pick $2^16$, 2 ALMs?
SuRF: point vs. mem, range, batch insert, trie height, FPR
B+tree: point vs. mem, range, insert, batch insert, profile
ART, HOT (optional depending on space): point vs. mem, range, insert, batch insert, trie height


\subsection{The Order-Preserving Encoding Model}
\label{sec:model}

An \emph{alphabet} $\Sigma$ of size $n$ is a symbol set
$\{s_0, s_1, \dots, s_{n-1}\}$ with a strict total ordering.
Without losing generality, let's assume $s_0 < s_1 < \dots < s_{n-1}$.

A \emph{string} $\vec s$ is a \emph{finite} sequence of symbols,
each picked from $\Sigma$.
The null string (i.e., with lenght zero) is denoted as $\epsilon$.

A \emph{variable-length string set} $\Sigma^*$ is the set of
all possible strings over $\Sigma$.
$\Sigma^*$ is countably infinite.
We use the \emph{lexicographical ordering} for $\Sigma^*$.
This ordering is total, not well-founded (and thus not well-ordered),
and not dense.
$\Sigma^*$ is a also \emph{free monoid} on $\Sigma$, with
\emph{concatenation} as the binary operation,
and $\epsilon$ as the identity element.

A \emph{morphism} $\phi$ maps one monoid $X$ to another monoid $Y$
and preserves the common binary operation $\cdot$. That is 
$\phi: X \rightarrow Y$ such that
$\phi(x_1 \cdot x_2) = \phi(x_1) \cdot \phi(x_2)$
and $\phi(\epsilon_X) = \phi(\epsilon_Y)$.
A monoid is a set that is closed under a single associative binary operation
and has an identity element.
In our case, the binary operation for any $\Sigma^*$
is string concatenation.

A (source) code is a function $C: \Sigma_1 \rightarrow \Sigma_2^*$.
A coding function $\phi: \Sigma_1^* \rightarrow \Sigma_2^*$
is defined inductively as
$\phi(s_i) = C(s_i)$ for $s_i \in \Sigma_1$,
and $\phi (s_{i_0} s_{i_1} \dots s_{i_k}) 
= \phi(s_{i_0}) \phi(s_{i_1}) \dots \phi(s_{i_k})$,
for $s_{i_j} \in \Sigma_1, 0 \le j \le k$.
$\phi$ is a morphism.
A code is order-preserving if
$\forall \vec s_1, \vec s_2 \in \Sigma_1^*,
\vec s_1 < \vec s_2 \implies \phi (\vec s_1) < \phi (\vec s_2)$.
The code is uniquely decodable if $\phi$ is injective.
Note that $\phi$ is not necessarily bijective.
In fact, we can prove the following theorem.

%% An order-preserving encoding is an \emph{injection}
%% $\phi: \Sigma_{1}^{*} \rightarrow \Sigma_{2}^{*}$ such that
%% $\forall s_1, s_2 \in \Sigma_{1}^{*} \implies \phi (s_1) < \phi (s_2)$.
%% We call $\Sigma_{1}^{*}$ the \emph{original space}
%% and $\Sigma_{2}^{*}$ the \emph{code space}.
%% Note that $\phi$ is not necessarily a \emph{bijection}, although
%% $\Sigma_{1}^{*}$ and $\Sigma_{2}^{*}$ have the same cardinality.
%% In fact, we can prove the following theorem.

\begin{theorem}
\label{thm:1}
There exists an order-preserving bijective code between
$\Sigma_1$ and $\Sigma_2$ if and only if $|\Sigma_1| = |\Sigma_2|$.
\end{theorem}

\begin{proof}
The backward direction can be proved by relabeling all the symbols
in $\Sigma_1$ with the corresponding symbols in $\Sigma_2$.

We prove the forward direction by contradiction.
It is equivalent to prove: if $|\Sigma_1| \ne |\Sigma_2|$,
there does not exist an order-preserving bijective code between
$\Sigma_1$ and $\Sigma_2$.
And it is sufficient to prove the $|\Sigma_1| < |\Sigma_2|$ case.

Let $|\Sigma_1| = m$, $|\Sigma_2| = n$, $m < n$.
Let $\Sigma_1 = \{s_0, s_1, \dots, s_{m-1}\}$,
where $s_0 < s_1 < \dots < s_{m-1}$,
and $\Sigma_2 = \{t_0, t_1, \dots, t_{n-1}\}$,
where $t_0 < t_1 < \dots < t_{n-1}$.

Suppose there exists an order-preserving bijective
code $C: \Sigma_1 \rightarrow \Sigma_2^*$ for $m < n$.
Because the code is bijective, we know that $\phi$
has an inverse function $\phi^{-1}: \Sigma_2^* \rightarrow \Sigma_1^*$.

Suppose $\phi^{-1}(t_j) = s_i \vec s$, $t_j \in \Sigma_2, s_i \in \Sigma_1$.
We show that $\vec s$ must be an empty string by contradiction.
Assume $\vec s \ne \epsilon$. Then $s_i < s_i \vec s$ in lexicographical order.
Since $\phi$ is order-preserving (i.e., strictly increasing),
$\phi(s_i) < \phi (s_i \vec s) = t_j$.
That means $\phi(s_i) = t_{j-k} \vec t_1$ for some $0 < k \le j$.
However, by definition, $\phi(s_i \vec s) = \phi(s_i) \phi(\vec s)
= t_{j-k} \vec t_1 \phi(\vec s) < t_j$. Contradiction.
Therefore, $\vec s = \epsilon$.
In other words, $\phi^{-1}(t_j) = s_i$ for any $t_j \in \Sigma_2$.
It shows that there is an injection from $\Sigma_2$ to $\Sigma_1$.
This contradicts with our assumption that $n > m$.
\end{proof}

Common source codes such as Huffman code and Arithmatic code
choose $\Sigma_2 = {0, 1}$.
In the order-preserving case, the Hu-Tucker code is an optimal
(i.e., with minimal expected length) prefix code over
alphabet $\Sigma_2 = {0, 1}$.

We define a funtion $f$ that maps a string to a rational number
between 0 and 1 (closed on 0).
That is $f: \Sigma^{*} \rightarrow \mathbb{Q} \cap [0, 1)$.
$f$ works as follows.
We map each $s_i$ in $\Sigma$, $i = 0, 1, \dots, n-1$, to a fixed
distinct rational number $q_i \in \mathbb{Q} \cap [0, 1)$ such that
$\epsilon = q_0 < q_1 < \dots < q_{n-1} < 1 = q_n$.
where $\epsilon > 0$ and can be arbitrarily small.
Let $l_i = q_{i+1} - q_i$.
For a string $str = s_{i_0} s_{i_1} \dots s_{i_{m-1}}$,
\begin{equation}
\begin{aligned}
f(str) &= q_{i_0} + \sum_{k=1}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t}) \\
&= q_{i_0} + q_{i_1}l_{i_0} + q_{i_2}l_{i_0}l_{i_1} + \dots + q_{i_{m-1}}l_{i_0}l_{i_1} \dots l_{i_{m-2}}
\end{aligned}
\end{equation}

\begin{lemma}
\label{lemma1}
In the above expression, for any $1 \le p \le m-1$.
\[
\sum_{k=p}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t}) < \prod_{t=0}^{p-1} l_{i_t}
\]
\end{lemma}

\begin{proof}
Prove by induction.
The base case is $p = m - 1$.
$q_{i_{m-1}} \prod_{t=0}^{m-2} l_{i_t} < \prod_{t=0}^{m-2} l_{i_t}$
because $q_{i_{m-1}} < 1$.

The inductive step: suppose the inequality holds for $p$.
For $p-1$, 
\begin{equation}
\begin{aligned}
\sum_{k=p-1}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t})
&= q_{i_{p-1}} \prod_{t=0}^{p-2} l_{i_t} + \sum_{k=p}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t}) \\
&< q_{i_{p-1}} \prod_{t=0}^{p-2} l_{i_t} + \prod_{t=0}^{p-1} l_{i_t} \\
&= (q_{i_{p-1}} + l_{i_{p-1}}) \prod_{t=0}^{p-2} l_{i_t} \\
&= q_{i_{p-1} + 1} \prod_{t=0}^{p-2} l_{i_t}
< \prod_{t=0}^{p-2} l_{i_t}
\end{aligned}
\end{equation}
\end{proof}

\begin{lemma}
\label{lemma2}
$f$ is an order-preserving bijection.
\end{lemma}

\begin{proof}
We first show that $f$ is an order-preserving injection.
That is $\forall str_1, str_2 \in \Sigma^{*}, str_1 < str_2 \rightarrow f(str_1) < f(str_2)$.
Let $str_1 = s_{i_0} s_{i_1} \dots s_{i_{m-1}}$,
$str_1 = s_{j_0} s_{j_1} \dots s_{j_{n-1}}$,
In lexicographical ordering, $str_1 < str_2$ if 
\begin{itemize}
\item either $str_1$ is a prefix of $str_2$, that is
$m < n$ and $s_{i_p} = s_{j_p}$ for any $p < m$.
\item or $s_{i_p} < s_{j_p}$ for the first $p$ where
$s_{i_p}$ and $s_{j_p}$ differ.
\end{itemize}

Case 1: $str_1$ is a prefix of $str_2$. Then,
$f(str_2) - f(str_1) = \sum_{k=m}^{n-1} (q_{j_k} \prod_{t=0}^{k-1} l_{j_t}) > 0$

Case 2: $s_{i_p} < s_{j_p}$ for the first $p$ where
$s_{i_p}$ and $s_{j_p}$ differ. Then,
\begin{equation}
\begin{aligned}
& f(str_2) - f(str_1) \\
& = \sum_{k=p}^{n-1} (q_{j_k} \prod_{t=0}^{k-1} l_{j_t}) 
- \sum_{k=p}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t}) \\
& = (q_{j_p} - q{i_p}) \prod_{t=0}^{p-1} l_{i_t}
- \sum_{k=p+1}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t})
+ \sum_{k=p+1}^{n-1} (q_{j_k} \prod_{t=0}^{k-1} l_{j_t}) \\
\end{aligned}
\end{equation}
Since $q_{j_p} > q_{i_p}$, $q_{j_p} - q_{i_p} > l_{i_p}$. Thus,
\begin{equation}
\begin{aligned}
& f(str_2) - f(str_1) \\
& > l_{i_p} \prod_{t=0}^{p-1} l_{i_t}
- \sum_{k=p+1}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t})
+ \sum_{k=p+1}^{n-1} (q_{j_k} \prod_{t=0}^{k-1} l_{j_t}) \\
& = \prod_{t=0}^{p} l_{i_t}
- \sum_{k=p+1}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t})
+ \sum_{k=p+1}^{n-1} (q_{j_k} \prod_{t=0}^{k-1} l_{j_t}) \\
\end{aligned}
\end{equation}
By~\cref{lemma1},
$\prod_{t=0}^{p} l_{i_t} > \sum_{k=p+1}^{m-1} (q_{i_k} \prod_{t=0}^{k-1} l_{i_t})$.
therefore, the above expression $> 0$.
Hence, we have proved that $f$ is an order-preserving injection.

Now because both $\Sigma^{*}$ and $\mathbb{Q} \cap [0, 1)$ are
countably infinite set, they have the same cardinality.
In this case, an injection between the two sets implies bijection.
\end{proof}

\begin{theorem}
For any two variable-length string sets $\Sigma_{1}^{*}$ and $\Sigma_{2}^{*}$,
there exists an order-preserving bijection
$g: \Sigma_{1}^{*} \rightarrow \Sigma_{2}^{*}$.
\end{theorem}

\begin{proof}

\end{proof}




\subsection{Fast Dictionary Encoding}
\label{sec:dictionary}

Dictionary layout

Concatenate algorithm: integer buffer

SIMD speed-up

batch encoding optimization

\subsection{Order-Preserving Huffman Codes}
\label{sec:ophc}

What codes to use? Criteria:
1. order-preserving
2. small dictionary

Hu-Tucker Algorithm

Discussion: OPHC is close to the optimal uniquely decodable codes.
But do we need unique decodability? Interesting future work

